Explaining Hyperparameter Optimization via Partial Dependence Plots

Automated hyperparameter optimization (HPO) can support practitioners to obtain peak performance in machine learning models. However, there is often a lack of valuable insights into the effects of different hyperparameters on the final model performance. This lack of explainability makes it difficult to trust and understand the automated HPO process and its results. We suggest using interpretable machine learning (IML) to gain insights from the experimental data obtained during HPO with Bayesian optimization (BO). BO tends to focus on promising regions with potential high-performance configurations and thus induces a sampling bias. Hence, many IML techniques, such as the partial dependence plot (PDP), carry the risk of generating biased interpretations. By leveraging the posterior uncertainty of the BO surrogate model, we introduce a variant of the PDP with estimated confidence bands. We propose to partition the hyperparameter space to obtain more confident and reliable PDPs in relevant sub-regions. In an experimental study, we provide quantitative evidence for the increased quality of the PDPs within sub-regions.

==> latex-math/ml-automl.tex <==


% lambdav
\newcommand{\lambdav}{\bm{\lambda}}											% lambda vector



==> latex-math/ml-bagging.tex <==
% ml - bagging, random forest

\newcommand{\bl}[1]{b^{[#1]}(x)}											% baselearner with argument for m
\newcommand{\blm}{\bl{m}}												    % baselearner without argument for m
\newcommand{\blmh}{\hat{b}^{[m]}(x)}										% estimated base learner 
\newcommand{\fM}{f^{[M]}(x)}                    % ensembled predictor
\newcommand{\fMh}{\hat f^{[M]}(x)}                    % estimated ensembled predictor
\newcommand{\ambifM}{\Delta\left(\fM\right)}          % ambiguity/instability of ensemble


==> latex-math/ml-bayesopt.tex <==
% ml - Bayesian Optimization

\newcommand{\minit}{m_{\text{init}}											% Size of the initial design
\newcommand{\lambdai}{\lambda^{[i]}											% input for black box optimization 
\newcommand{\lambdaopt}{\lambda^{*}}											% Minimum of the black box function Psi
\newcommand{\metadata}{\left\{\left(\lambdai, \Psi^{[i]}\right)\right\}}		% Metadata for the Gaussian process
\newcommand{\lambdavec}{\left(\lambda^{[1]}, \dots, \lambda^{[\minit]}\right)}  % Vector of different inputs


% \newcommand{\metadata}



\newcommand{\gp}{\mathcal{GP}\left(m(x), k\left(x, x'\right)\right)} 								% Gaussian Process 


==> latex-math/ml-boosting.tex <==
% ml - boosting
\newcommand{\fm}{f^{[m]}}                                                   % prediction in iteration m
\newcommand{\fmh}{\hat{f}^{[m]}}                                            % prediction in iteration m
\newcommand{\fmd}{f^{[m-1]}}                                                % prediction m-1
\newcommand{\fmdh}{\hat{f}^{[m-1]}}                                         % prediction m-1
\newcommand{\bmm}{b^{[m]}}                                                  % basemodel m
\newcommand{\bmmh}{\hat{b}^{[m]}}                                           % basemodel m with hat
\newcommand{\betam}{\beta^{[m]}}                                            % weight of basemodel m
\newcommand{\betamh}{\hat{\beta}^{[m]}}                                     % weight of basemodel m with hat
\newcommand{\betai}[1]{\beta^{[#1]}}                                        % weight of basemodel with argument for m
\newcommand{\errm}{\text{err}^{[m]}}                                        % weighted in-sample misclassification rate
\newcommand{\wm}{w^{[m]}}                                                   % weight vector of basemodel m
\newcommand{\wmi}{w^{[m](i)}}                                               % weight of obs i of basemodel m
\newcommand{\thetam}{\theta^{[m]}}                                          % parameters of basemodel m
\newcommand{\thetamh}{\hat{\theta}^{[m]}}                                   % parameters of basemodel m with hat
\newcommand{\rmm}{\tilde{r}^{[m]}}                                                  % pseudo residuals
\newcommand{\rmi}{\tilde{r}^{[m](i)}}                                               % pseudo residuals
\newcommand{\Rtm}{R_{t}^{[m]}}                                              % terminal-region
\newcommand{\Tm}{T^{[m]}}                                                   %
\newcommand{\ctm}{c_t^{[m]}}                                                % mean, terminal-regions
\newcommand{\ctmh}{\hat{c}_t^{[m]}}                                         % mean, terminal-regions with hat
\newcommand{\ctmt}{\tilde{c}_t^{[m]}}                                       % mean, terminal-regions
\newcommand{\fxk}{f_k(x)}                                                   % f_k(x)
\newcommand{\Lp}{L^\prime}
\newcommand{\Ldp}{L^{\prime\prime}}
\newcommand{\Lpleft}{\Lp_{\text{left}}}


==> latex-math/ml-feature-sel.tex <==
% ml - feature selection

\newcommand{\xjNull}{x_{j_0}}
\newcommand{\xjEins}{x_{j_1}}
\newcommand{\xl}{\mathbf{x}_l}
\newcommand{\pushcode}[1][1]{\hskip\dimexpr#1\algorithmicindent\relax} % IGNORE_NOTATION


==> latex-math/ml-gp.tex <==
% ml - Gaussian Process

\newcommand{\gp}{\mathcal{GP}\left(m(\bm{x}), k\left(\bm{x}, \bm{x}^\prime\right)\right)} 								% Gaussian Process Definition	
\newcommand{\mvec}{\mathbf{m}}												    						% Gaussian process mean vector
\newcommand{\Kmat}{\mathbf{K}}																			% estimated base learner 
\newcommand{\ls}{\ell}                                           % length-scale


==> latex-math/ml-lm.tex <==
\newcommand{\thx}{\thetab^T \xv}												% linear score: theta^T x



==> latex-math/ml-nn.tex <==
% ml - NNs
\newcommand{\neurons}{z_1,\dots,z_M} % vector of neurons

\newcommand{\hidz}{\mathbf{z}}                            % vector of hidden activations
\newcommand{\biasb}{\mathbf{b}}                           % bias vector

\newcommand{\biasc}{c}                          % bias in output


\newcommand{\wtw}{\mathbf{w}}                             % weight vector (general)

\newcommand{\Wmat}{\mathbf{W}}                             % weight vector (general)


\newcommand{\wtu}{\mathbf{u}}                             % weight vector of output neuron
%


% deeplearning - regularization
\newcommand{\Oreg}{\mathnormal{R}_{reg}(\theta|X,y)}				% regularized objective function
\newcommand{\Ounreg}{\mathnormal{R}_{emp}(\theta|X,y)}			% unconstrained objective function
\newcommand{\Pen}{\Omega(\theta)}							% penalty
\newcommand{\Oregweight}{\mathnormal{R}_{reg}(w|X,y)}			% regularized objective function with weight 
\newcommand{\Oweight}{\mathnormal{R}_{emp}(w|X,y)}				% unconstrained objective function with weight
\newcommand{\Oweighti}{\mathnormal{R}_{emp}(w_i|X,y)}			% unconstrained objective function with weight w_i
\newcommand{\Oweightopt}{\mathnormal{J}(w^*|X,y)}				% unconstrained objective function withoptimal  weight
\newcommand{\Oopt}{\hat{\mathnormal{J}}(\theta|X,y)}				% optimal objective function 
\newcommand{\Odropout}{\mathnormal{J}(\theta, \mu|X,y)}	           	% dropout objective function

% deeplearning - optimization
\newcommand{\Loss}{L(y, f(\xv, \thetab))}
\newcommand{\Lmomentumnest}{L(\yi, f(x^{(i)}, \thetab + \varphi \nub))}                  % momentum risk
\newcommand{\Lmomentumtilde}{L(\yi, f(x^{(i)}, \tilde{\thetab}))}                  % Nesterov momentum risk
\newcommand{\Lmomentum}{L(\yi, f(x^{(i)}, \thetab))} 
\newcommand{\Hess}{\mathbf{H}}
\newcommand{\nub}{\boldsymbol{\nu}}

% deeplearning - autoencoders
\newcommand{\uauto}{L(x,g(f(x)))}			% undercomplete autoencoder objective function
\newcommand{\dauto}{L(x,g(f(\tilde{x})))}		% denoising autoencoder objective function

% deeplearning - adversarials 
\newcommand{\deltab}{\boldsymbol{\delta}}
\newcommand{\Lossdeltai}{L(\yi, f(\xi + \deltab|\thetab))}
\newcommand{\Lossdelta}{L(y, f(\xv + \deltab| \thetab))}


==> latex-math/ml-rf.tex <==
% ml -  ensemble methods, random forest

\newcommand{\betam}{\beta^{[m]}}												% baselearner with argument for m
\newcommand{\betaM}{\beta^{[M]}}												% baselearner with argument for M
\newcommand{\betai}{\beta^{[1]}}												% baselearner with argument for 1


==> latex-math/ml-survival.tex <==
\newcommand{\Ti}[1][i]{T^{(#1)}}
\newcommand{\Ci}[1][i]{C^{(#1)}}  
\newcommand{\oi}[1][i]{o^{(#1)}}  
\newcommand{\ti}[1][i]{t^{(#1)}}  
\newcommand{\lambdai}[1][i]{\lambda^{(#1)}}  
\newcommand{\deltai}[1][i]{\delta^{(#1)}}  
\newcommand{\Lxdi}{L\left(\bm{\delta}, \fx\right)}           



==> latex-math/ml-svm.tex <==
% ml - svms
\newcommand{\sv}{\operatorname{SV}}                                         % supportvectors
% already defined in basic-math:
\newcommand{\HS}{\Phi}                                               % H, hilbertspace
\renewcommand{\sl}{\zeta}
\newcommand{\slvec}{\left(\zeta^{(1)}, \zeta^{(n)}\right)}		% slack variables (SVM)
\newcommand{\sli}{\zeta^{(i)}}																% slack variable (SVM)


\newcommand{\alphah}{\hat{\alpha}}													% alpha-hat
\newcommand{\alphav}{\bm{\alpha}}													% vector alpha (bold)
\newcommand{\alphavh}{\hat{\bm{\alpha}}}													% vector alpha-hat



\newcommand{\phix}{\phi(\xv)}          												% \phi(x)
\newcommand{\phixt}{\phi(\tilde \xv)}        										% \phi(x-tilde)



==> latex-math/ml-trees.tex <==
% ml - trees, extra trees

\newcommand{\Np}{\mathcal{N}}												% (Parent) node N
\newcommand{\Npk}{\Np_k}														% node N_k
\newcommand{\Nl}{\Np_1}														% Left node N_1
\newcommand{\Nr}{\Np_2}														% Right node N_2
\newcommand{\pikN}{\pi_k^{(\Np)}}                                           		% class probability node N
\newcommand{\pikNh}[1][k]{\hat\pi_#1^{(\Np)}}                                           % estimated class probability node N
\newcommand{\pikNlh}[1][k]{\hat\pi_#1^{(\Nl)}}
\newcommand{\pikNrh}[1][k]{\hat\pi_#1^{(\Nr)}}


==> latex-math/probmodel.tex <==


% gaussians
\newcommand{\muk}{\bm{\mu_k}}  

